Modality Selection and Skill Segmentation via Cross-Modality Attention

Incorporating additional sensory modalities such as tactile and audio into foundational robotic models poses significant challenges due to the curse of dimensionality. This work addresses this issue through modality selection. We propose a cross-modality attention (CMA) mechanism to identify and selectively utilize the modalities that are most informative for action generation at each timestep. Furthermore, we extend the application of CMA to segment primitive skills from expert demonstrations and leverage this segmentation to train a hierarchical policy capable of solving long-horizon, contact-rich manipulation tasks.

==> text/problem_statement.tex <==
\section{Problem Statement}


We aim to improve the sample efficiency of a multi-modal visuomotor policy which takes as input camera observation, contact observation, and proprioceptive observation to predict an action.

Formally we formulate the manipulation task as a Partially Observable Markov Decision Process (POMDP), which is a 7-tuple $\mathcal{M} = ( \mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R}, \Omega, \mathcal{O}, \gamma)$. In RPL, we begin with a base policy $\pi: \Omega \longrightarrow \mathcal{A}$ and try to learn a residual policy $f_\theta(\Bar{o})$ on a superset of observation $\Bar{\Omega}$, where $\Omega \subset \Bar{\Omega}$ to create an improved policy $\pi_\theta(\Bar{o}) = \pi(o) + f_\theta(\Bar{o})$\cite{silver2019residualpolicylearning}. This creates a new POMDP $\mathcal{M^{(\pi)}} = ( \mathcal{S}, \mathcal{A}, \mathcal{T^{(\pi)}}, \mathcal{R}, \Bar{\Omega}, \mathcal{O^{(\pi)}}, \gamma)$, where 
$$\mathcal{T}^{(\pi)}(\Bar{o}, a, \Bar{o'}) = \mathcal{T}(\Bar{o}, \pi(o) + a, \Bar{o'})$$


